The BLAST Observatory: A Sensitivity Study for Far-IR Balloon-borne Polarimeters

Sensitive wide-field observations of polarized thermal emission from interstellar dust grains will allow astronomers to address key outstanding questions about the life cycle of matter and energy driving the formation of stars and the evolution of galaxies. Stratospheric balloon-borne telescopes can map this polarized emission at far-infrared wavelengths near the peak of the dust thermal spectrum - wavelengths that are inaccessible from the ground. In this paper we address the sensitivity achievable by a Super Pressure Balloon (SPB) polarimetry mission, using as an example the Balloon-borne Large Aperture Submillimeter Telescope (BLAST) Observatory. By launching from Wanaka, New Zealand, BLAST Observatory can obtain a 30-day flight with excellent sky coverage - overcoming limitations of past experiments that suffered from short flight duration and/or launch sites with poor coverage of nearby star-forming regions. This proposed polarimetry mission will map large regions of the sky at sub-arcminute resolution, with simultaneous observations at 175, 250, and 350 $\mu m$, using a total of 8274 microwave kinetic inductance detectors. Here, we describe the scientific motivation for the BLAST Observatory, the proposed implementation, and the forecasting methods used to predict its sensitivity. We also compare our forecasted experiment sensitivity with other facilities.

==> sanity_check_table.tex <==
\begin{table}[]
\vspace{-0.2in}
     \scriptsize
    \centering
    \begin{tabular}{lcr}
        \toprule
        \textbf{Parameter} & \textbf{Value} &  \textbf{Notes}\\
        \midrule
        \multicolumn{3}{l}{\textbf{Input parameters}} \\
        $T$ & 300 K & assigned to ``warm'' components\\
        $\nu_0$ & 860 GHz & from model filter half-power points\\
        $\Delta \nu$ & 260 GHz & from model filter half-power points\\
        $t_{cold}$ & 0.27 & from model filters\\
        $t_{warm}$ & 0.96 & from model atmosphere, mirrors, window\\
        $\epsilon_{warm}$ & 0.04 & from model atmosphere, mirrors, window\\
        $(A\Omega/\lambda_0^2)$ & 1 & $\lambda_0 = c/\nu_0$ \\
        $R$ & 0.8 m & from Table X\\
        $FWHM$ & 55 arcseconds & from Table X \\
        $N_{det}$ & 1682 & from Table X\\
        $Yield$ & 0.8 & from Table X \\
        \cline{1-3}
        \multicolumn{3}{l}{\textbf{Performance parameters}} \\
        $P$ & $11 \, pW$ &  equation~\ref{eq:power_approx_2}  \\
        $NEP_{phot}$ & $1.1 \times 10^{-16} \, W Hz^{-0.5}$ & equation~\ref{eq:NEP_approx} \\
        $NEFD_{phot}$ & $59 \, mJy \, s^{0.5}$ & equation~\ref{eq:NEFD_approx} \\
        $\sigma_{I}$ & $0.020 \, MJy \, SR^{-1}$ & equation~\ref{eq:mapping_speed_total_intensity_approx_2} \\                
        $\sigma_{P}$ & $0.029 \, MJy \, SR^{-1}$ & equation~\ref{eq:mapping_speed_polarized_intensity_approx} \\

        \cline{1-3}

        \bottomrule
        
    \end{tabular}
    \caption{\small The approximate calculation - input parameters and results.}
    \label{tab:sanity_check}
\end{table}
